Learning Smooth State-Dependent Traversability from Dense Point Clouds

A key open challenge in off-road autonomy is that the traversability of terrain often depends on the vehicle's state. In particular, some obstacles are only traversable from some orientations. However, learning this interaction by encoding the angle of approach as a model input demands a large and diverse training dataset and is computationally inefficient during planning due to repeated model inference. To address these challenges, we present SPARTA, a method for estimating approach angle conditioned traversability from point clouds. Specifically, we impose geometric structure into our network by outputting a smooth analytical function over the 1-Sphere that predicts risk distribution for any angle of approach with minimal overhead and can be reused for subsequent queries. The function is composed of Fourier basis functions, which has important advantages for generalization due to their periodic nature and smoothness. We demonstrate SPARTA both in a high-fidelity simulation platform, where our model achieves a 91\% success rate crossing a 40m boulder field (compared to 73\% for the baseline), and on hardware, illustrating the generalization ability of the model to real-world settings. Our code will be available at https://github.com/neu-autonomy/SPARTA.

==> sections/experiment/simulation/obstacle_row.tex <==
% \begin{wraptable}{r}{0.4\textwidth}
%     \centering
%     \vspace{-0.15in}
%     \footnotesize
%     \begin{tabular}{c | c | c c}
%         \hline
%         Algorithm & $\alpha$ & S.R. $\uparrow$ & F (N) $\downarrow$ \\
%         \hline
%         \multirow{2}{2em}{Ours} &   0.9 &   \textbf{95}    &   \underline{450.19}  \\
%                                 &   0   &   89             &   \textbf{432.26}     \\
%         \hline
%         \multirow{2}{4em}{\textit{AngleInput}}  &   0.9 &   \underline{92} &   492.61              \\
%                                 &   0   &   89             &   548.91              \\
%         \hline
%         \textit{Elev}                    &   --  &   73             &   740.04              \\
%         \hline
%     \end{tabular}
%     \caption{Success Rate (S.R.) and Average Force (F) experienced by wheel nodes in simulation. Our model outperforms 
%     the baselines \textit{AngleInput} and \textit{Elev}. The performance of the models decrease when we ablate CVaR with mean. Best
%     result is \textbf{Bolded}, and second best is \underline{underlined}.}
%     \label{tab:exp:obs_belt}
%     \vspace{-0.15in}
% \end{wraptable}
\begin{wraptable}{r}{0.4\textwidth}
    \centering
    \vspace{-0.15in}
    \footnotesize
    \begin{tabular}{c | c | c c}
        \hline
        Algorithm & $\alpha$ & Suc. $\uparrow$ & Dmg. $\downarrow$ \\
        \hline
        \multirow{2}{2em}{Ours} &   0.9 &   \textbf{95}    &   \textbf{5}  \\
                                &   0   &   89             &   11          \\
        \hline
        \multirow{2}{4em}{AngleInput}  &   0.9 &   \underline{92} &   \underline{8}              \\
                                &   0   &   89             &   11              \\
        \hline
        Elev                    &   --  &   73             &   27              \\
        \hline
    \end{tabular}
    \caption{Number of success (Suc.) and vehicle damage (dmg.) in simulation. Our model outperforms 
    \textit{AngleInput} and \textit{Elev}. The performance of the models decrease when we ablate CVaR with mean. \textbf{Best}
    , \underline{Second best}.}
    \label{tab:exp:obs_belt}
    \vspace{-0.15in}
\end{wraptable}

In this experiment, we test our model's ability to identify safe traversal points and angles of approach
in a row of packed, randomly placed obstacles.
%
We consider two baselines, the \textit{AngleInput} and a heuristic baseline that chooses the point with lowest maximum elevation
under vehicle's wheel footprint (\textit{Elev}).
%
Since the obstacles are placed on flat ground, the \textit{Elev} baseline is equivalent to finding the plan with
lowest stepping difficulty as in~\citep{fan2021step, lee2025trg}.
% %
% We spawn a row of packed, randomly rotated and scaled obstacles in a narrow passage way between
% two walls (lethal obstacle), and thus force the vehicle to traverse the obstacle row in order to
% reach the goal placed on the other side of the obstacles.
% %
% The size of the obstacles is set to approximately $0.5m \times 0.5m \times 0.35m$ (slightly larger than 
% vehicle tire width and lower than vehicle ground clearance).
% %
% The grid resolution for elevation map and precomputed Fourier coefficients are set to 0.2m
% for all experiments in simulation.
% %
% A successfully traversal means the vehicle crossed the obstacles without damaging, and reaches
% the goal within the maximum steps allowed.
% %
% Besides the \textit{AngleInput} baseline, we include another baseline that selects the point/angle that induces
% the lowest elevation below the vehicle's wheel footprint (\textit{Elev}).
%
As shown in \cref{tab:exp:obs_belt}, our model achieves higher success rate (S.R., the vehicle drives over the obstacle without
damage) than the \textit{AngleInput}, but both learning-based method significantly outperforms \textit{Elev}.
%
This is expected because the obstacles are spawned with similar sizes, and as a result \textit{Elev} degenerates to random selection, 
leading to much lower success rate and thus high risk of vehicle damage.
% %
% As mentioned in \cref{sec:exp:data_collection}, we choose to predict tire deformation as a surrogate to vehicle damage.
% %
% The validity of this choice is demonstrated in the results because high risk of vehicle damage correlates with
% higher force, i.e., we observe the \textit{Elev} baseline induces much higher force on wheel nodes compared to the 
% other candidates.
%
When we ablate the inclusion of CVaR during planning by setting $\alpha=0$, which is equivalent to using 
the mean of the predicted distribution, the performance of both our model and \textit{AngleInput} dropped.
%
This is because the CVaR accounts for tail risk distribution and is thus more suitable for safety-critical tasks.



==> sections/experiment/simulation/simulation.tex <==
% \subsubsection{Traversing a Row of Obstacles}\label{sec:exp:row}
% \subfile{obstacle_row}

% \subsubsection{Crossing a Boulder Field}
% \subfile{boulder_field}

==> sections/experiment/traversability.tex <==
Explain augmenting EVORA pipeline with the additional information of heading angle, and compare testing results
on e.g., EMD2 test loss and planning conservativeness

==> sections/method/problem.tex <==
Given a terrain patch represented as a point cloud $\mathbf{P}$ captured by
depth sensor and processed by upstream mapping modules (e.g. Simultaneous 
Localization and Mapping~\citep{chen2023dliom, dong2024lidar}),
we are interested in modeling a real value function $\Gamma$ that captures the
target risk metric $\gamma \in \mathbb{R}$ associated with traversing it
\footnote{Examples of such metrics include risk of vehicle damage and terrain traction.}.
%
Note that we observe that such metric should be dependent on the angle of approach 
$\phi \in [0, 2\pi]$.
As a result, the function can be concretely written as 
$\Gamma: \mathbf{P} \times \phi \rightarrow \gamma$.
